Noisy intermediate-scale quantum (NISQ) algorithms

A universal fault-tolerant quantum computer that can solve efficiently problems such as integer factorization and unstructured database search requires millions of qubits with low error rates and long coherence times. While the experimental advancement towards realizing such devices will potentially take decades of research, noisy intermediate-scale quantum (NISQ) computers already exist. These computers are composed of hundreds of noisy qubits, i.e. qubits that are not error-corrected, and therefore perform imperfect operations in a limited coherence time. In the search for quantum advantage with these devices, algorithms have been proposed for applications in various disciplines spanning physics, machine learning, quantum chemistry and combinatorial optimization. The goal of such algorithms is to leverage the limited available resources to perform classically challenging tasks. In this review, we provide a thorough summary of NISQ computational paradigms and algorithms. We discuss the key structure of these algorithms, their limitations, and advantages. We additionally provide a comprehensive overview of various benchmarking and software tools useful for programming and testing NISQ devices.

==> Tables/OLD_TABLE.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*} 
\centering
% \begin{adjustbox}{width=\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{l l}
\hline 
\hline
Application  & Proposed implementation \\
\hline 
Hamiltonian ground state problem (\secref{sec:VQE}) &  \cite{peruzzo2014variational,mcclean2016theory,wecker2015progress}
\cite{kokail2019self}
\cite{wang2019accelerated}
\cite{liu2019variational}
\cite{garcia2018addressing}
\cite{lee2018generalized}
\cite{grimsley2019adaptive}
\cite{stair2020multireference}
\cite{ryabinkin2018qubit}
\cite{ryabinkin2020iterative}
\cite{lang2020iterative}
\cite{evangelista2019exact}
\cite{kottmann2020feasible}
\cite{kottmann2020reducing}
\cite{sokolov2020quantum}
\cite{barkoutsos2018quantum}
\cite{kandala2017hardware}
\cite{choquette2020quantum}
\cite{zhang2020mutual}

\\
\hline 
Hamiltonian excited states (\secref{sec:var_excited}) &  \cite{peruzzo2014variational,ryabinkin2018constrained}
\cite{higgott2019variational,lee2018generalized,tilly2020computation,jones2019variational}
\cite{mcclean2017hybrid,colless2018computation,takeshita2020increasing,stair2020multireference}
\cite{nakanishi2019subspace}
\cite{parrish2019quantum}
\cite{santagati2018witnessing}\\
\hline 
Hamiltonian Simulation (\secref{sec:hamilton_simulation})& \cite{li2017efficient,mcardle2019variational,yuan2019theory,endo2020variational,yoshioka2020variational,kubo2020variational}
\cite{heya2019subspace}
\cite{cirstoiu2020variational}
\cite{commeau2020variational}
\cite{bharti2020quantum}\\
\hline 
Imaginary Time Evolution & \cite{bharti2020quantum}, \cite{motta2020determining, mcardle2019variational}, \cite{sun2020quantum}  \\

\hline
Open system Simulation (\secref{sec:OpenQuantumSystem})& \cite{koppenhofer2020quantum,hu2020quantum}
\cite{yoshioka2020variational,endo2020variational,yuan2019theory,liu2020solving}\\
\hline 
Nonequilibrium steady state (\secref{sec:nonequilibrium})& \cite{kreula2016non}, \cite{yoshioka2020variational}, \cite{endo2020calculation}, \cite{jaderberg2020minimum}\\
\hline
Quantum computer-aided designs (\secref{sec:quantum_aided_design}) & \cite{kyaw2020quantum}, \cite{kottmann2020quantum}\\
\hline
Supervised Learning & \cite{perez2020data} \cite{schuld2019quantum,havlivcek2019supervised, kusumoto2019experimental}\cite{farhi2018classification, mitarai2018quantum,schuld2018quantum, schuld2019quantum,havlivcek2019supervised, schuld2020circuit}\cite{li2018quantum} \\
\hline 

Unsupervised Learning &  \cite{benedetti2017quantum}\\
\hline 
Reinforcement Learning & \cite{chen2020variational,lockwood2020reinforcement,lockwoodplaying}\cite{crawford2016reinforcement}\cite{lamata2017basic}\cite{cardenas2018multiqubit}\cite{albarran2020reinforcement} \\
\hline 
Quantum Foundations &  ~\cite{kirby2019contextuality,kirby2020contextual,arrasmith2019variational}\\
\hline 
Quantum Metrology (\secref{sec:quantum_metrology})&  ~\cite{koczor2020variational,kaubruegger2019variational,ma2020adaptive,beckey2020variational,meyer2020variational}\\
\hline 
Gibbs State Preparation (\secref{sec:gibbsstate})&  \cite{endo2020variational,chowdhury2020variational,haug2020generalized}\\
\hline 
Quantum Linear System Problem (\secref{sec:linear_system_problem})& \cite{huang2019nearterm,bravo2019variational,xu2019variational2}\\
\hline 
Singular Value Decomposition (\secref{subsec: SVD})& ~\cite{bravo2020quantum,wang2020variational} \\
\hline 
Nonlinear Differential Equations (\secref{sec:nonlinear_differential})&  \cite{lubasch2020variational,kyriienko2020solving,gaitan2020finding,haug2020generalized} \\
\hline 
Error Mitigation & \cite{li2017efficient}\cite{temme2017error}\cite{temme2017error}\cite{mcclean2017hybrid,colless2018computation,mcardle2019error,sagastizabal2019experimental,mcclean2020decoding,barron2020preserving} \cite{bonet2018low,mcardle2019error,sagastizabal2019experimental}\cite{otten2019accounting}\\
\hline 
Error Correction (\secref{sec:variational_error_correction})&  \cite{johnson2017qvector,xu2019variational2}\\
\hline 
Combinatorial Optimization (\secref{sec:optimization})&   \cite{arute2020quantum} \cite{bengtsson2020improved,vikstaal2020applying}\cite{cook2019quantum}\cite{fingerhuth2018quantum}\cite{grandrive2019knapsack}\cite{oh2019solving}\cite{choi2020quantum,saleem2020max}~\cite{garcia2018addressing}\cite{perdomo2012finding}\\
\hline 
Factoring (\secref{sec:factoring})& \cite{anschuetz2019variational,karamlou2020analyzing} \\
\hline 
Problems in Finance (\secref{sec:finance})&  \cite{egger2020quantum,bouland2020prospects,orus2019quantum,marzec2016portfolio,rosenberg2016solving,venturelli2019reverse,cohen2020portfolio}\\
\hline 
Quantum Circuit Compilation ()&  \\
\hline 
Nuclear physics (\secref{sec:nuclear_physics})& \cite{avkhadiev2020accelerating}\cite{liu2020quantum}\cite{dumitrescu2018cloud,lu2019simulations}\cite{roggero2020quantum} \\
\hline 
Quantum Cloning & \cite{coyle2020variational}\\
\hline 
Fidelity Estimation (\secref{sec:fidelity_estimation})&  \cite{cerezo2020fidelity}\\
\hline 
Quantum Control (\secref{sec:quantum_optimal_control}) & \cite{li2017hybrid,dive2018situ,lu2017enhancing,policharla2020algorithmic} \\
\hline
\end{tabular}}
% \end{adjustbox}
\caption{Table of NISQ Algorithms. References with $\ast$ are experimental realizations.} 
\label{tab:Applications}
\end{table*}

==> conventions.tex <==

\section*{CONVENTIONS}

See \url{https://cdn.journals.aps.org/files/styleguide-pr.pdf} for some notation and figure and table styles.

\subsection{Mathematical relations and quantities}

\begin{itemize}
    \item Matrices: capital latin letters (check subsection bellow to see if the letter is taken already for a particular quantity)
    \item Vectors (use "boldsymbol"): $\boldsymbol{v}$
    \item Unit vectors: $\boldsymbol{\hat{v}}$
    \item Vector components: $(v_{x},v_{y},v_{z})$
    \item Operators use "hat" (not quantum gates or hamiltonians): $\hat{h}$
    \item Order: $O$ as in $O(n^2)$.
    \item Use of "mathcal": sets? Like dataset?
    \item Use of "mathbb":
    \item Use upper greek:
    \item Use lower greek: 
    \item Use italic: quantum gates ($CNOT$, $S$, $H$,...), acronym definition (\textit{Variational Quantum Eigensolver} (VQE)?,...
    \item "paragraph" and italic title as next level after "subsubsection".
\end{itemize}

\begin{itemize}
    \item latin indices order: $i,j,k,l,$?
    \item greek indices?
\end{itemize}

\begin{itemize}
    \item Pauli matrix $a$ ($a=x,y,z$) acting on qubit $i$: $\sigma_{a}^{i}$
    \item Pauli vector ($=(\sigma_{x},\sigma_{y},\sigma_{z})$): $\boldsymbol{\sigma}$
    \item Pauli string: $\hat{P}$
    \item Hamiltonian (not to be confused with Hadamard gate): $H$
    \item Hamiltonian subsystem $i$: $h_{i}$
    \item Hamiltonian coefficient: $c_{i}$
    \item Hadamard gate: $H_{d}$
    \item Hilbert space: $\mathcal{H}$
    \item Identity: $I$
    \item Real, Complex, whole numbers: $\mathbb{R}$, $\mathbb{C}$, $\mathbb{W}$
    \item Real and Imaginary parts: 
    \item Bit string: $z$
    \item Paulis gates vs Paulis spin chain: ($X$, $Y$, $Z$) vs $(\sigma_{x},\sigma_{y},\sigma_{z})$
    \item epsilon error: $\epsilon$
    \item perturbation: $\delta$
\end{itemize}

\begin{itemize}
    \item Number of qubits: $n$
    \item Dimension of Hilbert space of $n$ qubits: $N=2^n$
    \item Number of qubits lesser than $n$: $m$
    \item Local dimension: $d$
    \item General quantum state: $|\psi\rangle$
    \item Ground state:
    \item Time: $t$
    \item Adiabatic step: $s$
    \item Coefficient wavefunction:
    \item Computational basis element $i$ (for more than 1 qubit): $|e_{i}\rangle$
    \item Superposition of computational basis states: $|D\rangle$
    \item General parameterized state: $\ket{\Psi(\boldsymbol{\theta})}$
    \item Gate $S$ applied to a particular qubit $i$: $S^{(i)}$?
    \item Probability measurement state $|i\rangle$: $p_{i}$
    \item Probability measurement state $|i\rangle$ on qubit $a$: \com{$p_{i}^{(a)}$?}
    \item Expectation value operator $\mathcal{O}$: $\langle \hat{O} \rangle$
    \item State $|i\rangle$ applied to $n$ qubits: $|i\rangle^{\otimes n}$,
    \item Partial derivative w.r.t $\theta_{i}$: $\partial_{i}$ (defined in \eqref{eq:gradient}).
    \item Time derivative: $\dot{\theta}$
\end{itemize}

Particular letters taken: $H$, $S$ (quantum gates/hamiltonian/hilbert space), $p$ (probability)

\subsection{Particular quantities}
\begin{itemize}
    \item Objective function: $\hat{O}$
    \item Loss function (Same as objective?):
    \item Fidelity: $F$
    \item general function: $f$
    \item Data set: $\mathcal{D}$
    \item Train and test sets:
    \item State preparation circuit: $P$
    \item Encoding circuit: $E$
    \item General PQC: $U$
    \item Total quantum circuit: $\mathcal{U}$
    \item Measurement gate: $M$
    \item Parameter set 1 PQC: $\boldsymbol{\theta}$
    \item Parameter set 2 PQC: $\boldsymbol{\phi}$
    \item Initial parameters: $\boldsymbol{\theta_{0}}$
    \item Problem Hamiltonian: $H_{P}$
    \item Mixing Hamiltonian: $H_{M}$
    \item Fubini-Study Metric: $\mathcal{F}$
\end{itemize}
